MetroGNN: Metro Network Expansion with Reinforcement Learning

Selecting urban regions for metro network expansion to meet maximal transportation demands is crucial for urban development, while computationally challenging to solve. The expansion process relies not only on complicated features like urban demographics and origin-destination (OD) flow but is also constrained by the existing metro network and urban geography. In this paper, we introduce a reinforcement learning framework to address a Markov decision process within an urban heterogeneous multi-graph. Our approach employs an attentive policy network that intelligently selects nodes based on information captured by a graph neural network. Experiments on real-world urban data demonstrate that our proposed methodology substantially improve the satisfied transportation demands by over 30\% when compared with state-of-the-art methods. Codes are published at https://github.com/tsinghua-fib-lab/MetroGNN.

==> related.tex <==
\section{Related Work}

\noindent\textbf{Deep Reinforcement Learning for Planning.}
Deep reinforcement learning (DRL)~\citep{mnih2015human} approaches, which combines RL algorithms with deep neural networks (DNN) as function approximators, have demonstrated excellent performance and become the new state-of-the-art, especially in complex planning tasks such as gaming~\citep{mnih2013playing,silver2016mastering,ye2020mastering}, autonomous driving~\citep{kiran2021deep,li2022path,shi2020drone}, natural language processing~\citep{li2016deep,he2015deep,tan2022roberta}, recommender system~\citep{zheng2018drn,zhao2018deep,wang2021reinforcement}, and solving mathematical problems~\cite{fawzi2022discovering,bello2016neural,bengio2021machine}.
On the one hand, the efficient approximators such as DQN~\citep{mnih2013playing,mnih2015human} can accurately handle high-dimensional inputs.
On the other hand, the actor-critic framework~\citep{konda1999actor} is effective in narrowing down the action space and improving exploration efficiency.


\noindent\textbf{Transportation Network Design.}
As a widely studied engineering task~\citep{guihaire2008transit,ibarra2015planning,farahani2013review,kepaptsoglou2009transit,laporte2011planning,wang2021deep}, existing solutions to this problem can be classified into three primary categories: mathematical programming methods, heuristic methods, and deep reinforcement learning methods.
Mathematical programming methods\citep{escudero2009approach,wang2023designing,gutierrez2013rapid,owais2021design} typically formulate it as an Integer Linear Programming (ILP) problem and then apply a solver to find the optimal solution.
For example, \citet{wei2019strategic} applied the minimum distance to the utopia point to handle the bi-objective Mixed-Integer Linear Programming (MILP) problem.
However, the computational complexity increases drastically as the problem scales up, making it challenging to find optimal solutions within a reasonable time limit.
Heuristic methods, including Tabu Search~\citep{dufourd1996locating,fan2008tabu}, Simulated Annealing~\citep{fan2006using,kumar2020novel,zhao2006optimization}, and Evolutionary Algorithms~\citep{mumford2013new,arbex2015efficient,chakroborty2003genetic,nayeem2018solving,bourbonnais2021transit}, have also emerged to address this problem.
However, it is difficult to handle the diverse constraints of metro networks with suitable heuristic operators, and these methods often invest substantial time in exploring impractical solutions.
Recently, \citet{wei2020city} explored the usage of RL for metro line planning.
However, they ignore the complicated features, and the adopted grid-like city representation induces significant errors from real-world scenarios.




